MARTSIA: Enabling Data Confidentiality for Blockchain-based Process Execution

Multi-party business processes rely on the collaboration of various players in a decentralized setting. Blockchain technology can facilitate the automation of these processes, even in cases where trust among participants is limited. Transactions are stored in a ledger, a replica of which is retained by every node of the blockchain network. The operations saved thereby are thus publicly accessible. While this enhances transparency, reliability, and persistence, it hinders the utilization of public blockchains for process automation as it violates typical confidentiality requirements in corporate settings. In this paper, we propose MARTSIA: A Multi-Authority Approach to Transaction Systems for Interoperating Applications. MARTSIA enables precise control over process data at the level of message parts. Based on Multi-Authority Attribute-Based Encryption (MA-ABE), MARTSIA realizes a number of desirable properties, including confidentiality, transparency, and auditability. We implemented our approach in proof-of-concept prototypes, with which we conduct a case study in the area of supply chain management. Also, we show the integration of MARTSIA with a state-of-the-art blockchain-based process execution engine to secure the data flow.

==> tables/experiments.tex <==
\begin{tabular}{@{} l S[table-format=5.2] S[table-format=10.0] S[table-format=1.5] S[table-format=5.0] S[table-format=10.0] S[table-format=1.5] S@{}}
	\toprule
	                   &               \multicolumn{3}{c}{\texttt{setIPFSInfo}}                &            \multicolumn{3}{c}{\texttt{setUserInfo}}             &                   \\ \cmidrule(lr){2-4}\cmidrule(lr){5-7}
	 & \textbf{gasUsed}    & \textbf{gasPrice}  & \textbf{Total cost} & \textbf{gasUsed}    & \textbf{gasPrice}  & \textbf{Total cost} & \textbf{ETH/EUR}  \\
	                   & \textbf{{[}unit{]}} & \textbf{{[}wei{]}} & \textbf{{[}EUR{]}}  & \textbf{{[}unit{]}} & \textbf{{[}wei{]}} & \textbf{{[}EUR{]}}  & \textbf{exchange} \\ \midrule
	avg.               & 67486.52            & 1399400015         & 0.16438             & 40755               & 1370810611         & 0.09734             & 1746.35           \\
	min                & 67484.6             & 1000000007         & 0.12378             & 40755               & 1000000007         & 0.07475             & 1650.68           \\
	max                & 67487               & 1649000034         & 0.18587             & 40755               & 1644053019         & 0.11191             & 1834.14           \\ \bottomrule
\end{tabular}

==> tables/message-decoding.tex <==
\begin{tabular}{|l|l|l|}
\hline
Header 
& Plain Key 
& Body \\ \hline

\lstinputlisting[firstline=1,lastline=4]{code/header.txt}	&  
\lstinputlisting[firstline=1,lastline=1]{code/symmetric_keys.txt}	& \lstinputlisting[firstline=1,lastline=3]{code/body.txt}     \\ 
	\cline{1-1}\cline{2-2}\cline{3-3}
	
\lstinputlisting[firstline=7,lastline=11]{code/header.txt}	
&	\lstinputlisting[firstline=3,lastline=3]{code/symmetric_keys.txt}       
&    \lstinputlisting[firstline=5,lastline=10]{code/body.txt}  \\ 
\cline{1-1}\cline{2-2}\cline{3-3}
  \lstinputlisting[firstline=14,lastline=18]{code/header.txt}       &   \lstinputlisting[firstline=5,lastline=5]{code/symmetric_keys.txt}     &  \lstinputlisting[firstline=12,lastline=16]{code/body.txt}    \\ \hline
\end{tabular}


==> tables/message-encoding-metadata.tex <==
\begin{tabular}{|l|l|l|}
\hline
Metadata 
& Header 
& Body \\ \hline

	& \lstinputlisting[firstline=1,lastline=4]{code/header.txt} 
	& \lstinputlisting[firstline=1,lastline=3]{code/body.txt}     \\ 
	\cline{2-2}\cline{3-3}
	
\lstinputlisting[firstline=1,lastline=2]{code/metadata.txt}	
&	\lstinputlisting[firstline=7,lastline=11]{code/header.txt}       
&    \lstinputlisting[firstline=5,lastline=10]{code/body.txt}  \\ 
\cline{2-2}\cline{3-3}
         &  \lstinputlisting[firstline=14,lastline=18]{code/header.txt}      &  \lstinputlisting[firstline=12,lastline=16]{code/body.txt}    \\ \hline
\end{tabular}


==> tables/message-encoding-short.tex <==
\begin{tabular}{|c|l|l|l|}
\hline
   Message
 & Original Data
 & Access Policy
 & Symmetric Key \\ \hline
  
 & \lstinputlisting[firstline=9,lastline=11]{code/original_data.txt}
 & \lstinputlisting[firstline=1,lastline=2]{code/access_policy.txt}
 & \lstinputlisting[firstline=1,lastline=1]{code/symmetric_keys.txt} \\ 
 \cline{2-2}\cline{3-3}\cline{4-4}
   \makecell{Bill \\ of \\ materials}
 & \lstinputlisting[firstline=13,lastline=18]{code/original_data.txt} 
 & \lstinputlisting[firstline=4,lastline=6]{code/access_policy.txt} 
 & \lstinputlisting[firstline=3,lastline=3]{code/symmetric_keys.txt} \\ 
 \cline{2-2}\cline{3-3}\cline{4-4} 
 & \lstinputlisting[firstline=20,lastline=24]{code/original_data.txt} 
 & \lstinputlisting[firstline=8,lastline=10]{code/access_policy.txt} 
 & \lstinputlisting[firstline=5,lastline=5]{code/symmetric_keys.txt} \\
 \hline
 
\end{tabular}%

==> tables/messages-plaintext-withkeys.tex <==
\begin{tabular}{|c|l|l|}
\hline
   Message
 & Original data
 & Encryption/decryption key \\ 
 \hline
 
   \makecell{Supply purchase order \\ (ramp)}
 & \lstinputlisting[firstline=1,lastline=4]{code/original_data.txt}
 & \lstinputlisting[firstline=1,lastline=1]{code/symmetric_keys.txt}\\ 
 \hline
   
 & \lstinputlisting[firstline=8,lastline=16]{code/original_data.txt} 
 & \lstinputlisting[firstline=3,lastline=3]{code/symmetric_keys.txt} 
  \\ 
  \cline{2-2}\cline{3-3} 
  
   \makecell{Export document}
  & \lstinputlisting[firstline=18,lastline=22]{code/original_data.txt} 
 & \lstinputlisting[firstline=5,lastline=5]{code/symmetric_keys.txt} 
  \\ 
  \cline{2-2}\cline{3-3} 
  
& \lstinputlisting[firstline=24,lastline=26]{code/original_data.txt} 
 & \lstinputlisting[firstline=7,lastline=7]{code/symmetric_keys.txt} \\
 \cline{2-2}\cline{3-3} 
 
 & \lstinputlisting[firstline=28,lastline=32]{code/original_data.txt} 
 & \lstinputlisting[firstline=9,lastline=9]{code/symmetric_keys.txt} \\
 \hline
 
 \makecell{National \\ customs clearance}
& \lstinputlisting[firstline=36,lastline=40]{code/original_data.txt} 
 & \lstinputlisting[firstline=11,lastline=11]{code/symmetric_keys.txt} \\
 \hline

\end{tabular}

